Understanding Concurrent Transmissions: The Impact of Carrier Frequency Offset and RF Interference on Physical Layer Performance

The popularity of concurrent transmissions (CT) has soared after recent studies have shown their feasibility on the four physical layers specified by BLE 5, hence providing an alternative to the use of IEEE 802.15.4 for the design of reliable and efficient low-power wireless protocols. However, to date, the extent to which physical layer properties affect the performance of CT has not yet been investigated in detail. This paper fills this gap and provides an extensive study on the impact of the physical layer on CT-based solutions using IEEE 802.15.4 and BLE 5. We first highlight through simulation how the impact of errors induced by relative carrier frequency offsets on the performance of CT highly depends on the choice of the underlying physical layer. We then confirm these observations experimentally on real hardware and with varying environmental conditions through an analysis of the bit error distribution across received packets, unveiling possible techniques to effectively handle these errors. We further study the performance of CT-based data collection and dissemination protocols in the presence of RF interference on a large-scale testbed, deriving insights on how the employed physical layer affects their dependability.

==> experiments_testbed.tex <==
% !TEX root = main.tex

% Infrastructure description
\section{D-Cube Testbed} \label{sec:testbed}
\cb{This section will be split into smaller chunks and will go into the experimental setup of section 4 and 5.} 

\dcubee is a low-cost measurement tool that can accurately measure key performance metrics such as end-to-end delay, reliability, and power consumption in hardware.
Originally designed to support a dependability competition~\cite{schuss17competition} comparing the performance of state-of-the-art protocols under the same settings, \dcubee was recently opened to the public as an open benchmark~\cite{schuss20dcube} \dcubee is comprised of two main components: i) a low-cost testbed consisting of networked observer modules, each with several low-power wireless nodes (target nodes) attached, ii) {several services hosted on on-site servers - including backend systems, a command and control broker, and a frontend application. 
% Overview
%\begin{figure}[!tb]
%	\centering	
%	\vspace{-2.50mm}
%	\includegraphics[clip, trim=0.6cm 0.6cm 0.6cm 0.6cm,width=0.5\textwidth]{figures/tug/overview.pdf}
%	\vspace{-1.25mm}
%	\caption{\dcubee primary components and their communication protocols.}
%	\label{fig:tug_overview}
%	\vspace{-3.25mm}
%\end{figure}
%

\boldpar{Observer modules}
In order to measure and control a target node, \dcubee utilizes observer modules. Each of these modules is built around an off-the-shelf Raspberry Pi 3B~(\raspberry) with an additional custom energy and latency measurement PCB as well as a node multiplexer.
The \raspberry runs a real-time patched Linux kernel and it is used to communicate with the attached target nodes as well as with the backend server. The \raspberry uses an analog-to-digital converter (ADC) on a measurement PCB to simultaneously measure both voltage and current consumption of the attached target nodes. The measurement PCB also includes galvanic isolation to ensure that the \raspberry does not affect the energy measurements by isolating all GPIOs, reset, USB, I2C and the 5V USB power. Furthermore, the measurement PCB can be equipped with an optional GPS module to ensure better time synchronization as well as with a power over Ethernet (PoE) module to make it possible to directly power each observer module from the network infrastructure.
Each observer module can support up to four target nodes: a node multiplexer allows the selection of the target node to be used via software. This also ensures that the measurements are not affected by the inactive target nodes. Currently \dcubee is equipped with TelosB replicas and Nordic Semiconductors~nRF52840-DK target nodes.

\boldpar{Server infrastructure}
All observer modules are controlled by a backend that communicates with the \raspberry via the advanced message queueing protocol (AMQP). On top of this protocol, Remote Procedure Calls (RPC) are implemented, which allow the backend to utilize abstracted functions and to issue a single command to all observer modules (e.g., to program the correct firmware on all target nodes used in an experiment without any details on the required tools or memory layout of each individual node). This removes the need for observer modules to coordinate among each other and requires only the implementation of a set of high-level functions (e.g., the selection of a given target node, the ability to control power and reset on each target node, and the capability of starting and stopping the measurement service). Using a REST API, \dcubee users can queue a large number of experiments, which are then automatically scheduled by the infrastructure. This last feature, in particular, was extremely useful to gather the extremely large data sets presented within this paper.
%
%\subsection{Network Infrastructure}
%Under normal circumstances, the network infrastructure such as switches would be considered transparent to the testbed. However, in order to reduce the downtime of the testbed, the backend may power cycle observer modules in case of a non-recoverable error e.g., a kernel panic, by controlling the PoE state on any given switch port. This requires the backend to have a mapping between Observer Modules and switch ports.

\boldpar{Benchmark workflow}
% Workflow
\begin{figure}[!tb]
	\centering	
	\vspace{-2.50mm}
	\includegraphics[clip, trim=0.6cm 0.6cm 0.6cm 0.6cm,width=0.45\textwidth]{figures/tug/workflow.pdf}
	\vspace{-1.25mm}
	\caption{\dcubee's benchmark worflow.}
	\label{fig:tug_workflow}
	\vspace{-3.25mm}
\end{figure}
%
\dcubee has been explicitly designed to allow fully-automated benchmarking of protocol performance; taking a single firmware, and running it repeatedly under a wide range of settings. The general workflow, from uploading a binary firmware to the resulting output metrics, is illustrated in Figure~\ref{fig:tug_workflow}.
\dcubee uses so called \textit{benchmark suites}, which contain information such as node type, a set of layouts available and a description of the output metrics. Using the latter, a variety of metrics computed from the raw measurements e.g. the energy consumption of each node over time split into a setup and experiment phase, reliability of out-of-order communication, per packet as well as average latency.
While the benchmark suite describes the general setup, goal and available platform, each individual experiment may select from a range of other settings such as traffic load or generated RF interference. These settings are used to describe requirements for an application, e.g., communication of 30 bytes of periodic data in an environment co-located with \wifi.
%
\boldpar{Binary Patching}
To facilitate automated benchmarking of protocols, \dcubee employs a binary patching scheme~\cite{schuss18benchmark} to inject knowledge about current benchmark suite and experiment parameters directly into the firmware. The firmware file needs to be build with this feature in mind, placing a well-known data structure at a predefined address. This structure contains placeholders all variables modified by this benchmark suite, e.g., message size and period, a list of IDs for sources and destinations as well as the nodes own ID. Before flashing the firmware onto the target node by the observer module, a python script searches for a section in the binary which includes the predefined address and replaces the content of the data structure with the current experiments values. In addition, a user defined version can be enabled on-demand, which allows the binary patching to replace an additional structure containing firmware specific parameters, e.g., the PHY mode, data rate or number of retransmissions. Using binary patching, a single firmware can be used to explore a wide range of settings including different layouts, message sizes and periods, in addition to firmware specific parameters such as PHY settings with minimal effort by queueing a large set of experiments using \dcubee's REST API. This REST API also allows to download serial logs as well as performance metrics after completion.
%
\boldpar{Repeatable RF interference}
To enable the generation of controllable and repeatable RF interference \jamlabng~\cite{schuss19jamlabng} has been integrated into D-Cube. \jamlabng is a framework based on Nexmon~\cite{nexmon:project}, a C-based firmware patching framework for Broadcom/Cypress \wifi chips found on Raspberry Pi Zero W, 3B,3B+ and 4B. This enables \jamlabng to run directly on the ARM CPU on this \wifi chip without being affected by the OS or network stack on the Raspberry Pi. \dcubee's integration of \jamlabng generates testbed wide interference using four key parameters: interference duration, period, power and channel. 
In this paper, we use Intensive interference (Jamming 3), which uses all channels, with each RPI choosing and staying on a different channel. The interference lasts for approx. 8ms every 13ms at a power of 200mW. The mild interference (Jamming 2) utilizes a reduced power of 30mW and duration of approx. 5ms with the same 13ms period\ms{Are these descriptions sufficient of is more detail required here?}.
%
